Efficient Method for Finding Optimal Strategies in Chopstick Auctions with Uniform Objects Values

We propose an algorithm for computing Nash equilibria (NE) in a class of conflicts with multiple battlefields with uniform battlefield values and a non-linear aggregation function. By expanding the symmetrization idea of Hart [9], proposed for the Colonel Blotto game, to the wider class of symmetric conflicts with multiple battlefields, we reduce the number of strategies of the players by an exponential factor. We propose a clash matrix algorithm which allows for computing the payoffs in the symmetrized model in polynomial time. Combining symmetrization and clash matrix algorithm with the double oracle algorithm we obtain an algorithm for computing NE in the models in question that achieves a significant speed-up as compared to the standard, LP-based, approach. We also introduce a heuristic to further speed up the process. Overall, our approach offers an efficient and novel method for computing NE in a specific class of conflicts, with potential practical applications in various fields.

==> parts/algorithm_clash_matrix.tex <==
\begin{algorithm}
\SetAlgoLined
\KwIn{Two non-increasing vectors $\aPure$ and $\bPure$}
\KwResult{Payoff value from given profile.}

\tcc{initialization}
Determine the clash matrix\;
Determine the array $knots[]$, containing pairs of coordinates of consecutive points at which the ``cut-off'' occurs, in ascending order\;
Allocate a $4$-dimensional array $values[]$, of size $2n \times (n+1) \times (n+1) \times (n+1)$\;

 \For{$knotIndex \leftarrow 0$ \KwTo $length(knots) - 1$}
 {
    $knot \leftarrow knots[knotIndex]$\;
    $i \leftarrow knot[0]$\;
    $j \leftarrow knot[1]$\;
    \For{$rooksNum \leftarrow 0$ \KwTo $\min(i,j)$}
    {
        \For{$k_W \leftarrow 0$ \KwTo $\min(i,j)$} 
        {
            \For{$k_L \leftarrow 0$ \KwTo $\min(i,j)$} %TODO tu chyba coś trzeba sprytniej iść po tych wartościach (chyba jednak nie)
            {
                $values[knotIndex, rooksNum, k_W, k_L] \leftarrow H(i,j,rooksNum,k_W,k_L)$\;
                 \tcc{function H uses $value[]$ and clash matrix}
            }
        }
    }
 }
 $lastKnot \leftarrow lenght(knots)-1$\; 
 \tcc{last knot is always $(n,n)$}
 $result = 0$\;
 \For{$k_W \leftarrow 0$ \KwTo $n$} 
{
    \For{$k_L \leftarrow 0$ \KwTo $n$} %TODO tu chyba coś trzeba sprytniej iść po tych wartościach (chyba jednak nie)
    {
        $result += values[lastKnot, n, k_W, k_L] \cdot f_n(k_W, k_L)$
    }
}
 \Return $result/factorial(n)$\;
 \caption{The dynamic algorithm for calculating payoff from a pair of symmetric strategies}
\end{algorithm}

==> parts/new_abstract.tex <==
We consider computations of Nash equilibria (NE) in a class of conflicts with multiple battlefields. Conflicts with multiple battlefields are zero-sum games with succinct representation: the number of strategies of each player is exponential with respect to the size of the game description. We propose homogeneous description of rivalry of two players that distribute discrete resources on a set of battlefields with uniform values. Individual battlefields are won by a player assigning more resources to given battlefield. Different methods of aggregating game outcome from individual battlefields outcomes yields different models -- many of which are well known in the literature. We show that regardless the aggregation function, the problem of computing NE can be reduced to the symmetrized model, that allows only symmetric strategies which involve mixing on all of the permutations of battlefields with uniform probability distribution. We propose a polynomial time algorithm for computing payoffs for symmetrized mixed strategy profiles for the whole class of models and use the Multiplicative Weights Update algorithm for computing $\epsilon$-equilibria of the games. These methods allow for computing significantly larger instances of the games than the LP based approach and are suitable for implementation on a computational cluster.

==> parts/table.tex <==
\begin{tabularx}{180pt}{|c|r|r|r|}
 \hline
 Res & Pure  & Symmetrized & Mult \\ 
 \hline
10  &  1961256  &  42  &  46696 \\
13  &  20058300  &  101  &  198597 \\
16  &  145422675  &  230  &  632272 \\
19  &  818809200  &  483  &  1695257 \\
22  &  3796297200  &  972  &  3905655 \\
25  &  15084504396  &  1861  &  8105590 \\
28  &  52860229080  &  3446  &  15339590 \\
31  &  166871334960  &  6158  &  27098300 \\
34  &  482320623240  &  10715  &  45013590 \\
 \hline


\end{tabularx}
